Specialization of Run-time Configuration Space at Compile-time: An Exploratory Study

Numerous software systems are highly configurable through run-time options, such as command-line parameters. Users can tune some of the options to meet various functional and non-functional requirements such as footprint, security, or execution time. However, some options are never set for a given system instance, and their values remain the same whatever the use cases of the system. Herein, we design a controlled experiment in which the system's run-time configuration space can be specialized at compile-time and combinations of options can be removed on demand. We perform an in-depth study of the well-known x264 video encoder and quantify the effects of its specialization to its non-functional properties, namely on binary size, attack surface, and performance while ensuring its validity. Our exploratory study suggests that the configurable specialization of a system has statistically significant benefits on most of its analysed non-functional properties, which benefits depend on the number of the debloated options. While our empirical results and insights show the importance of removing code related to unused run-time options to improve software systems, an open challenge is to further automate the specialization process.

==> images/tables.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{sidewaystable}
%\begin{table*}
\scriptsize
\caption{The average and standard deviation of %+ 1 standard deviation 
\textit{encoding time} in seconds [s] of $8$ videos by the baseline ($S_0$) and specialized systems ($S_1-S_{20}$)}
\label{tbl:encodingtime}
\begin{tabular}{p{1.1cm}p{0.4cm}|p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}r|r|p{0.01cm}p{3.1cm}}
\cmidrule(r){1-13} \cmidrule(l){15-15}
System 
& Unit
& ultrafast  
& superfast    
& veryfast    
& faster   
& fast    
& medium  
& slow   
& slower   
& veryslow   
& placebo 
& $H_{03}$
&
& Encoding time
\\   \cmidrule(r){1-13}
$S_0$ 
& [s]
& $0.28 \pm 0.02$
& $0.48 \pm 0.01$ 
& $0.74 \pm 0.03$ 
& $1.03 \pm 0.04$ 
& $1.41 \pm 0.04$ 
& $1.73 \pm 0.04$ 
& $2.76 \pm 0.08$ 
& $4.97 \pm 0.16$ 
& $9.85 \pm 0.37$ 
& $35.03 \pm 0.72$ 
& 
&
& $(mean \pm std)$
\\ \cline{1-13} \cline{15-15} 
$S_1$  
& [s]
& - 
& - 
& - 
& - 
& $1.39 \pm 0.03$ 
& $1.77 \pm 0.05$ 
& $2.85 \pm 0.10$  
& $5.08 \pm 0.18$
& $9.86 \pm 0.26$ 
& $35.32 \pm 0.46$ 
& 
&
& $S_0: (5.83 \pm 10.67)$
\\
$S_2$  
& [s]
& - 
& - 
& $0.67 \pm 0.02$ 
& $0.96 \pm 0.01$ 
& $1.29 \pm 0.02$ 
& $1.63 \pm 0.04$ 
& $2.61 \pm 0.06$ 
& $4.78 \pm 0.18$ 
& $9.27 \pm 0.42$ 
& $33.23 \pm 0.69$ 
& 
&
& $Avr. S_{1-10}: (5.82 \pm 10.61)$
\\
$S_3$  
& [s]
& - 
& $0.46 \pm 0.02$ 
& $0.73 \pm 0.02$ 
& $1.02 \pm 0.02$  
& $1.43 \pm 0.03$ 
& $1.79 \pm 0.05$  
& $2.80 \pm 0.06$  
& $5.00 \pm 0.18$ 
& $9.96 \pm 0.26$ 
& $35.34 \pm 0.76$ 
& 
&
& $Avr. S_{11-20}: (5.51 \pm 10.22)$
\\
$S_4$  
& [s]
& -  
& $0.46 \pm 0.01$ 
& $0.73 \pm 0.01$ 
& $1.03 \pm 0.01$ 
& $1.43 \pm 0.03$ 
& $1.78 \pm 0.05$  
& $2.92 \pm 0.10$  
& $5.07 \pm 0.19$ 
& $10.11 \pm 0.32$ 
& $35.09 \pm 0.48$ 
& 
&
& $Avr. S_{1-20}: (5.77 \pm 10.54)$
\\ \cline{15-15} 
$S_5$ 
& [s]
& $0.29 \pm 0.01$
& $0.46 \pm 0.02$ 
& $0.75 \pm 0.01$ 
& $1.06 \pm 0.03$  
& $1.46 \pm 0.04$  
& $1.83 \pm 0.04$ 
& $2.87 \pm 0.08$ 
& $5.05 \pm 0.19$  
& $10.09 \pm 0.37$ 
& $35.20 \pm 0.63$ 
& 
&
& 
\\ 
$S_6$  
& [s]
& $0.30 \pm 0.01$ 
& $0.47 \pm 0.02$ 
& $0.75 \pm 0.02$ 
& $1.05 \pm 0.01$ 
& - 
& - 
& - 
& - 
& - 
& - 
& 
&
& Bitrate
\\
$S_7$  
& [s]
& $0.28 \pm 0.01$ 
& $0.45 \pm 0.01$ 
& - 
& - 
& - 
& - 
& - 
& - 
& - 
& -
& 
&
& $(mean \pm std)$
\\ \cline{15-15}
$S_8$  
& [s]
& $0.28 \pm 0.01$ 
& - 
& - 
& - 
& - 
& - 
& - 
& - 
& - 
& -
& 
&
& $S_0: (892.75 \pm 59.10)$
\\
$S_9$  
& [s]
& $0.29 \pm 0.02$ 
& -  
& - 
& - 
& - 
& - 
& - 
& - 
& - 
& - 
& 
&
& $Avr. S_{1-10}: (894.45 \pm 57.75)$
\\
$S_{10}$  
& [s]
& - 
& -  
& - 
& - 
& - 
& - 
& - 
& - 
& - 
& - 
& 
&
& $Avr. S_{11-20}: (901.28 \pm 54.47)$
\\ \cmidrule(r){1-13}
Avr. $S_{1-10}$ 
& [s]
& $0.29 \pm 0.01$ \textcolor{red}{$\uparrow$}  
& $0.46 \pm 0.01$ \textcolor{ao}{$\downarrow$} 
& $0.72 \pm 0.03$ \textcolor{ao}{$\downarrow$} 
& $1.02 \pm 0.04$ \textcolor{ao}{$\downarrow$} 
& $1.40 \pm 0.07$ \textcolor{ao}{$\downarrow$} 
& $1.76 \pm 0.08$ \textcolor{red}{$\uparrow$} 
& $2.81 \pm 0.12$ \textcolor{red}{$\uparrow$} 
& $4.99 \pm 0.13$ \textcolor{red}{$\uparrow$} 
& $9.86 \pm 0.34$ \textcolor{red}{$\uparrow$} 
& $34.84 \pm 0.90$ \textcolor{ao}{$\downarrow$} 
& \cellcolor{red!15}$\neg$R
&
& $Avr. S_{1-20}: (895.59 \pm 56.97)$
\\ \cmidrule(r){1-13} \cmidrule{15-15} 
$S_{11}$  
& [s]
& $0.29 \pm 0.01$ 
& - 
& - 
& - 
& - 
& - 
& - 
& - 
& - 
& -
& 
&
&
\\
$S_{12}$  
& [s]
& - 
& $0.47 \pm 0.02$ 
& - 
& - 
& - 
& - 
& - 
& - 
& - 
& -
& 
&
& Frame rate
\\
$S_{13,14}$  
& [s]
& - 
& - 
& $0.66 \pm 0.03$ 
& $0.95 \pm 0.03$ 
& - 
& - 
& - 
& -  
& - 
& - 
& 
&
& $(mean \pm std)$
\\ \cline{15-15}
$S_{15-20}$  
& [s]
& -  
& - 
& - 
& - 
& $1.24 \pm 0.04$ 
& $1.53 \pm 0.03$ 
& $2.56 \pm 0.07$ 
& $4.70 \pm 0.16$ 
& $9.21 \pm 0.40$ 
& $33.55 \pm 0.54$  
& 
&
& $S_0: (625.25 \pm 699.67)$
\\ \cmidrule(r){1-13}
Avr. $S_{11-20}$ 
& [s]
& $0.29 \pm 0.0$ \textcolor{red}{$\uparrow$} 
& $0.47 \pm 0.0$  \textcolor{ao}{$\downarrow$} 
& $0.66 \pm 0.0$ \textcolor{ao}{$\downarrow$} 
& $0.95 \pm 0.0$ \textcolor{ao}{$\downarrow$} 
& $1.24 \pm 0.0$ \textcolor{ao}{$\downarrow$} 
& $1.53 \pm 0.0$ \textcolor{ao}{$\downarrow$} 
& $2.56 \pm 0.0$ \textcolor{ao}{$\downarrow$} 
& $4.70 \pm 0.0$ \textcolor{ao}{$\downarrow$} 
& $9.21 \pm 0.0$ \textcolor{ao}{$\downarrow$} 
& $33.55 \pm 0.0$ \textcolor{ao}{$\downarrow$} 
& \cellcolor{green!15}R 
&
& $Avr. S_{1-10}: (625.24 \pm 703.25)$
\\  \cline{1-13} \cmidrule(r){1-13}
Avr. $S_{1-20}$ 
& [s]
& $0.29 \pm 0.01$  \textcolor{red}{$\uparrow$} 
& $0.46 \pm 0.01$ \textcolor{ao}{$\downarrow$} 
& $0.71 \pm 0.04$ \textcolor{ao}{$\downarrow$} 
& $1.01 \pm 0.05$ \textcolor{ao}{$\downarrow$} 
& $1.37 \pm 0.09$  \textcolor{ao}{$\downarrow$} 
& $1.72 \pm 0.12$  \textcolor{ao}{$\downarrow$} 
& $2.77 \pm 0.15$  \textcolor{red}{$\uparrow$} 
& $4.95 \pm 0.16$ \textcolor{ao}{$\downarrow$} 
& $9.75 \pm 0.41$ \textcolor{ao}{$\downarrow$} 
& $34.62 \pm 0.96$ \textcolor{ao}{$\downarrow$} 
& \cellcolor{green!15}R 
&
& $Avr. S_{11-20}: (653.84 \pm 688.23)$
\\ 
$\%$ of $S_{1-20}$ 
&
& \cellcolor{red!15}$1.39\%$ 
& \cellcolor{green!15}$-4.13\%$
& $-4.08\%$
& $-2.12\%$
& $-2.76\%$
& $-0.33\%$ 
& $0.31\%$
& $-0.49\%$ 
& $-1.07\%$
& $-1.18\%$ 
& 
&
& $Avr. S_{1-20}: (630.01 \pm 700.64)$
\\
\cmidrule(r){1-13} \cmidrule(l){15-15} 
\end{tabular}
\end{sidewaystable}
%
